Blocking Trails for $f$-factors of Multigraphs

Blocking flows, introduced by Dinic [2] for network flow, have been used to speed up many augmenting-path type algorithms, especially matching algorithms e.g., [18, 23, 16]. We present an $O(m)$ time algorithm for blocking trails for f-factors of general multigraphs. This improves a previous algorithm by a factor of $\alpha(m,n)$. This speeds up a number of efficient algorithms for f-factors, e.g., the algorithm of [11] for maximum weight f-matching improves by the aforementioned $\alpha(m,n)$ factor to running time $O( \sqrt {\Phi \log \Phi} m \log (\Phi W) )$ for $\Phi =\sum _{v\in V} f(v)$, $W$ the maximum edge weight. This time bound is within a factor $\sqrt {\log \Phi}$ of the bound for bipartite multigraphs. The technical difficulty for this work stems from the fact that previous algorithms for both matching and $f$-matching use vertex contractions to form blossoms, but our dfs-based approach necessitates using edge contractions. As an example difficulty, edge contractions introduce a new form of blossoms we call "skew blossoms". These are configurations that must be reorganized in order to become valid blossoms.

==> CLabelling.tex <==
Consider the moment in time when a blossom $B$ becomes complete,
i.e., $d(\eta(B))$ returns. Take any edge $xz$ incident to $B$,
say $x\in V(B) \not\ni z$. As an arc $e$ is either 
$xz$ or $zx$. Either

$e$ is in the current search path $SP$,
or
 
$e=zx$ and  $e=\eta(B)$, or

$e=xz$ and $xz$ descends from $B$ or $SP$ in $\o{\T.}$


==> dAlg.tex <==
\def\myif #1{{\sf {if}} (#1)}
\def\myelif #1{{\sf else if} (#1)}
\def\myifel #1 #2 #3 {{\sf if} (#1) {{#2}} {\sf else} {{#3}}}
\def\myelse {{\sf else}}

\def\myfor #1{{\sf for} (#1)} 
\def\mywhile #1{{\sf while} (#1)}
\def\myloop {{\sf loop}}

\def\mycom #1{{\tt /* {\hskip-3pt#1\hskip-3pt} */}}

\def\myand {{\sf and }}
\def\myor {{\sf or }}
\def\myto {{\sf to }}
\def\myreturn{{\sf return}}

\def\sm.{\mathy{\cal S^-}}

{\parindent=0pt

\bigskip

{\sf procedure} {find\_blocking\_set}

initialize \T. to an empty forest and \A. to an empty set
%,and all $b$ entries to $\emptyset$

initialize lists $GL(x)$ to $\delta(x)\cup \gamma(x)$
and $BL(x)$ to $\emptyset$

\bigskip

\myfor {$\alpha \in V(G)$}

{\hi

\myif {$def(\alpha)>0$ and no invocation $d(\vtx z\alpha)$ has returned}
%$\alpha$ was not the root of a previous  unsuccessful search}
$d(\vtx \varepsilon \alpha)$ 

\iffalse
\mywhile {$\exists$ a vertex $\alpha$, $def(\alpha)>0$,
$\alpha$ was not the root of a previous  unsuccessful search}
$d(\vtx \varepsilon \alpha)$ 
\fi

%{\hi

\mycom{$\varepsilon$ is an artificial vertex,
$\epsilon \alpha$ is a  matched artificial arc directed to $\alpha$}

}



{\sf return} \A.

\bigskip


{\sf procedure} {\em d}(\vtx zx)    %($e$)
%\mycom{$e$ is an edge of $G$ directed to vertex $x$}

%$x \gets$ the head of edge $e$, 

%$e\gets$ arc $zx$, $\mu \gets \mu(e)$
$\mu \gets \mu(zx)$


\bigskip

\myif {$def(x)>0$ \myand $\mu = \o M$ \myand 
$(x\ne \alpha$ \myor  $def(\alpha)\ge 2)$} 

{\hi 

\mycom{augment step}

add the $\o {\T.}$ path  from $\alpha$ to $x$ to \A.

terminate every currently executing invocation of  $d$, including this one
}

\bigskip

\mywhile {$\exists \text{ edge } xy\in GL(x) \cap \o \mu $}

{\hi

remove $xy$ from $GL(x)$ and $GL(y)$

\mycom{grow step} 

add an arc $xy$ to \T., originating at node $\vtx zx$; \mycom{\vtx xy is a leaf}

$B_{\vtx xy}\gets \{\vtx xy\}$

$d(\vtx xy)$

}
\bigskip


\myloop

{\hi

\mycom{blossom base test}

\myif {no occurrence of $x$ is in a blossom} 

{\hi



\myifel 
{$\exists \text{ edge } xy\in BL(x) \cap \o \mu $} %
{{$xy \gets {\rm pop}(BL(x))$}} {{\myreturn}}
}

\mycom{blossom enlarge test}

\myelif{\vtx zx or some descendant  \vtx wx is in a blossom} 
%{$\vtx zx$ is an internal node of \T.}
%$\vtx zx$ is in a blossom, i.e., $B_{\vtx zx}\ne \{\vtx zx\}$}

{\hi

\myifel{$\exists \text{ edge } xy\in BL(x)$} % 
{$xy \gets {\rm pop}(BL(x))$} {\myreturn}

}

\mycom{blossom step}

let $P$ be the path in $\o {\T.}$ from 
$B_\vtx z x$ to $B_{\vtx yx}$

\iffalse
\myfor {every node $v\in V(\T.)$ with $B_v\in P$} $b(v)\gets b(x,e)$
add $B_{\vtx v u}$ to $B_\vtx z x$

for every node v on an edge of P

\fi

\myfor {every arc $uv$  of $P$}
merge $B_{\vtx uv}$ into  $B_{\vtx zx}$

\myfor {every arc $uv$  of $P$, as ordered in $P$ but skipping the first arc}
\iffalse
\myfor {every arc $uv$  of $P$, as ordered in $P$, $u\ne \vtx zx$}
\mycom{blossom-invocation loop}
\fi

{\hi

\mycom{blossom-invocation loop}

$d(\vtx v u)$

}

}

\iffalse
\mywhile {$\exists$ a vertex of 
$P- \vtx yx -\vtx zx $ 
that has not been blossom scanned}

{\hi
$u \gets$ the first such vertex in 
$P- \vtx yx -\vtx zx $ 

%\mycom{by definition $x$ has been blossom scanned}

$uv\gets $  the arc leaving $u$ in $P$

$d(\vtx v u)$

\mycom{$u\in V(G)$ is blossom-scanned if $d(\vtx v u)$ returns}

%\vtx vu 

\mycom{(but not if $d(\vtx v u)$  is terminated)}

}

}
\fi

\bigskip

add $zx$ to $BL(x)$

\myreturn
}

\bigskip


\paragraph*{Elaboration of the algorithm}
Let us comment on some statements in the algorithm.
An invocation $d(\vtx \varepsilon \alpha)$
made in the main routine is called a {\em search (for an augmenting trail)}.
This invocation is terminated iff an augmenting trail is discovered.
So $d(\vtx \varepsilon \alpha)$ returns if no augmenting trail is discovered.
The discussion following Lemma \ref{PendantProp} 
will show $\alpha$ remains free for the rest of the algorithm.


We make some conventions to justify the terminology for \T..
As usual we call \T. a search tree even though it 
is a forest (each search starts at a different root).
Also we allow \T. to contain loops $xx$ (added in grow steps).
Similarly we allow the path $P$ in a blossom step 
to contain loops.

We continue discussing 
the blossom step.
In the blossom base test,
it is unclear why the pop routine returns the correct edge
(i.e., it may have the wrong M-type).
Lemma \ref{oMufirstRemoveLemma}
will show correctness.
In the blossom enlarge test note
\vtx zx is in a blossom is easily checked.
%since it means $B_{\vtx zx}\ne \{\vtx zx\}$.
%NO, BECAUSE OF SINGLETON BLOSSOMS
%but these gives nops anyway
Also let us informally explain this test (the
explanation is proved rigorously below).
The possibility that \vtx zx is in a blossom
covers ordinary blossoms (the possibility holds
when either \vtx zx is already the base vertex of a
blossom, or $zx$ or its reverse occurs on the blossom path).
The possibility that \vtx zx is not in a blossom
but \vtx wx is holds for skew blossoms.
%\vtx zx or some descendant  \vtx wx is in a blossom
%recall an internal node is non-leaf \cite{CLRS}.
Next note that in the blossom step
we identify each arc of $P$ by its nodes in  \T..
%The {\sf for} loops traverse the arcs of $P$ in path order.
\iffalse
For example in the {\sf while} loop, \vtx yx and \vtx zx are vertices of
$P$. Similarly in the loop that merges $B$-values, $v$ and $w$ are vertices of
$G$.
\fi
The blossom step may have $P$  empty, 
specifically $B_{\vtx yx}=B_{\vtx zx}$.
We call such a blossom step a {\em noop} since nothing changes
(there are no $B_{\vtx uv}$ merges or $d(\vtx vu)$ invocations).
An invocation $d(\vtx xy)$ in a grow step adds $xy$ to \T., but
$d(\vtx vu)$ in the blossom step does not cause a similar addition.
So the call chain of $d$ can be a proper subset of
the current search path.
(More precisely,
an invocation $d(\vtx zx)$ in the current call chain has
the corresponding arc $xz$ or $zx$
in the current search path. Within blossoms,
the call chain may omit search path edges.)

\paragraph*{Examples of the algorithm}
Fig.\ref{dExamplesFig} gives examples of searches of $d$.

MOVE THIS
Fig.\ref{bStepCasesFig} illustrates the three types of blossoms in $d$.

As illustrated in
Fig.\ref{bStepCasesFig}, at the moment the algorithm begins a blossom step, the base
base vertex has been blossom scanned; the atoms properly descending from
the base vertex have not been blossom scanned; lastly, in
Fig.\ref{bStepCasesFig}(b), vertex $s$ need not be blossom scanned and so 
can be $u_1$.
%This choice is important when the search is successful.





For more  motivation
let us explain the restriction on $uv$ in the blossom-invocation loop.
(The explanation gets rigorously proved in our analysis below.)
Let $B$ denote the blossom formed in the blossom step.
   Consider two cases.

Suppose  the first node of $P$ is not in a blossom.
This means 
$B$ is either the first blossom formed with base edge $zx$,
or $B$ is a skew blossom.
There
is no need to invoke $d(\vtx vu)$ because the edges of $GL(x)$
have all been scanned before the blossom step.
(For the first blossom case
the scanning occurs because of edges $zx$ and $yx$.
For the skew blossom case
the scanning occurs in the blossom with base edge $yx$.)

Suppose the first end of $P$ is in a blossom $B'$.
(We remark that this implies the last end of $P$ is also in $B'$.)
There is no need for $d(\vtx vu)$ since
\vtx vu belongs to $B'$. So just like the skew blossom case,
$B'$ gives an invocation
$d(\vtx wu)$ with 
$\vtx wu =\vtx vu$ and $\mu(wu)=\mu(vu)$.

\iffalse
A vertex $v\in V(B)$ is either a vertex in a contracted blossom, or a
vertex $u$ in the blossom-invocation loop, or the base vertex $\beta=\vtx zx$
of $B$ if $zx$ is not in a contracted blossom.  The $u$ vertices are
scanned in the corresponding recursive invocation $d(\vtx vu)$.
\fi





